Training-free Object Counting with Prompts

This paper tackles the problem of object counting in images. Existing approaches rely on extensive training data with point annotations for each object, making data collection labor-intensive and time-consuming. To overcome this, we propose a training-free object counter that treats the counting task as a segmentation problem. Our approach leverages the Segment Anything Model (SAM), known for its high-quality masks and zero-shot segmentation capability. However, the vanilla mask generation method of SAM lacks class-specific information in the masks, resulting in inferior counting accuracy. To overcome this limitation, we introduce a prior-guided mask generation method that incorporates three types of priors into the segmentation process, enhancing efficiency and accuracy. Additionally, we tackle the issue of counting objects specified through text by proposing a two-stage approach that combines reference object selection and prior-guided mask generation. Extensive experiments on standard datasets demonstrate the competitive performance of our training-free counter compared to learning-based approaches. This paper presents a promising solution for counting objects in various scenarios without the need for extensive data collection and counting-specific training. Code is available at \url{https://github.com/shizenglin/training-free-object-counter}

==> temp.tex <==
%Although SAM exhibits a general ability to segment various objects prompted by users, it lacks the specific capability to segment individual instances of subjects. Consequently, SAM cannot be directly employed for the counting task at hand.
 Lu et al. \cite{lu2019class} propose a method that utilizes a shared embedding module to extract feature maps from both query images and exemplars. These feature maps are then concatenated and passed through a learnable matching module, resulting in the generation of a similarity map. Yang et al. \cite{yang2021class} introduce a technique that performs feature comparison using dot product, which yields a more reliable density map compared to other similarity metrics. Ranjan et al. \cite{ranjan2021learning} enhance the reliability of the similarity map by employing multiscale augmentation during training and test-time adaptation. While these existing methods employ pre-trained networks for feature extraction or utilize fixed inner product-based similarity metrics, which can introduce noise in the similarity maps, Shi et al. \cite{shi2022represent} propose an end-to-end approach to jointly learn feature representations and similarity metrics, thereby addressing the problem of noisy similarity maps. In an alternative approach, You et al. \cite{you2023few} propose a similarity-aware feature enhancement method that combines the strengths of both feature representations and similarities, resulting in improved performance. Other problems have also been studied, such as inefficient test-time adaptation \cite{ranjan2022exemplar}, the requirement of human-annotated exemplars \cite{ranjan2022exemplar,xu2023zero}.


 %
\begin{table*}[!t]
\centering
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
&\multirow{2}{*}{\textbf{Training}} & \multirow{2}{*}{\textbf{Prompt}} & \multicolumn{4}{c}{\textbf{Validation Set}} & \multicolumn{4}{c}{\textbf{Testing Set}}\\
\cmidrule(lr){4-7} \cmidrule(lr){8-11}
& & & \textbf{MAE} &
\textbf{RMSE} & \textbf{NAE} &
\textbf{SRE} & \textbf{MAE} &
\textbf{RMSE} & \textbf{NAE} &
\textbf{SRE} \\
\hline
GMN \cite{lu2019class} &Yes&box&29.66 &89.81 &- &-&26.52 &124.57 &-&-\\
FamNet+ \cite{ranjan2021learning} &Yes&box&23.75 &69.07 &0.52 &\underline{4.25}&22.08 &99.54 &0.44&6.45\\
CFOCNet+ \cite{yang2021class} &Yes&box&21.19 &\underline{61.41} &- &-&22.10 &112.71 &-&-\\
BMNet+ \cite{shi2022represent} &Yes&box&\underline{14.68} &91.74 &\underline{0.27} &6.57&\underline{15.82} &\underline{58.41} &\underline{0.25}&\underline{2.74}\\
SAM &No&box&41.53 &106.58 &1.17 &7.82&42.48 &137.50 &1.14&8.13\\
SAM+similarity &No&box&34.39 &114.34 &0.50&5.26&26.29 &137.89 &0.38&4.38\\
\rowcolor{Gray}
Ours &No&box&\textbf{25.57} &\textbf{101.06} &\textbf{0.35} &\textbf{4.25}&\textbf{19.95} &\textbf{132.16} &\textbf{0.29}&\textbf{3.80}\\
\hline
SAM &No&point&- &- &- &-&- &- &-&-\\
SAM+similarity &No&point&- &- &- &-&- &- &-&-\\
\rowcolor{Gray}
Ours &No&point&- &- &- &-&- &- &-&-\\

\bottomrule
\end{tabular}}
\caption{\textbf{Effect of our approaches with point and box prompt on FSC-147.} \textbf{Bold} indicates the best counting results of training-free methods, and \underline{underline} indicates the best counting results of learning-based methods. 
}
\label{tab:fsc147}
\end{table*}

%
\begin{table*}[!t]
\centering
\resizebox{1.5\columnwidth}{!}{
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
&\multirow{2}{*}{\textbf{Training}} & \multicolumn{4}{c}{\textbf{FSC-147}} & \multicolumn{4}{c}{\textbf{CARPK}}\\
\cmidrule(lr){3-6} \cmidrule(lr){7-10}
& & \textbf{MAE} &
\textbf{RMSE} & \textbf{NAE} &
\textbf{SRE} & \textbf{MAE} &
\textbf{RMSE} & \textbf{NAE} &
\textbf{SRE} \\
\hline
Xu \etal \cite{xu2023zero} &Yes&26.93 &88.63 &0.36 &4.26&22.09 &115.17 &0.34&3.74\\
SAM &No&41.53 &106.58 &1.17 &7.82&42.48 &137.50 &1.14&8.13\\
SAM+similarity &No&- &- &- &-&- &- &-&-\\
\rowcolor{Gray}
Ours &No&\textbf{34.65} &\textbf{111.49} &\textbf{0.46} &\textbf{5.28}&\textbf{26.01} &\textbf{136.60} &\textbf{0.36}&\textbf{4.49}\\


SAFECount \cite{you2023few} &Yes&box&15.28 &\underline{47.20} &- &-&\underline{14.32} &85.54 &-&-\\

%Moreover, we provide results obtained by using the similarity map directly for our prior-guided mask generation approach, without utilizing our reference object selection algorithm to obtain high-quality similarity maps.

 These methods contribute to improving the quality and reliability of similarity maps through various techniques such as shared embedding \cite{lu2019class}, dot product-based comparisons \cite{yang2021class}, multiscale augmentation and test-time adaptation \cite{ranjan2021learning}, joint feature and similarity metric learning \cite{shi2022represent}, and similarity-aware feature enhancement \cite{you2023few}. Each approach addresses the limitations of previous methods and provides advancements in class-agnostic object counting.

 , which is computed by
\begin{equation}
M^{(k)} = \dfrac {F_I \cdot F_R^{(k)}} {\left\| F_I\right\| _{2}\left\| F_R^{(k)}\right\| _{2}}.
\label{eq:cos}
\end{equation}

%\MM{I dont understand this; what is the size of the reference object feature? did you convolution-like cosine similarity? with a sliding window?}
%\MM{this is really confusing; a lot of details missing; what is the sliding window size; what is the step size?}

\MM{we need to re-work this paragraph. I got what you meant; but the math does not tally. math notations are messy as well. n and N denote the number binary masks; then suddenly have m masks; what is m; the total number of object instances on the image regardless of classes? if so, say so}

%
\begin{table}[!t]
\centering
\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
&\multirow{2}{*}{\textbf{Training}} & \multirow{2}{*}{\textbf{Prompt}} & \multicolumn{4}{c}{\textbf{FSC-147}}\\
\cmidrule(lr){4-7}
& & & \textbf{MAE} $\downarrow$  &
\textbf{RMSE} $\downarrow$ & \textbf{NAE} $\downarrow$ &
\textbf{SRE} $\downarrow$ &  \\
\hline
GMN \cite{lu2019class} &Yes&box&26.52 &124.57 &-&-\\
FamNet+ \cite{ranjan2021learning} &Yes&box&22.08 &99.54 &0.44&6.45\\
CFOCNet+ \cite{yang2021class} &Yes&box&22.10 &112.71 &-&-\\
BMNet+ \cite{shi2022represent} &Yes&box&\underline{15.82} &\underline{58.41} &\underline{0.25}&\underline{2.74}\\
SAM &No&N.A.&42.48 &137.50 &1.14&8.13\\
Ours (vanilla) &No&box&26.29 &137.89 &0.38&4.38\\
\rowcolor{Gray}
Ours &No&box&\textbf{19.95} &\textbf{132.16} &\textbf{0.29}&\textbf{3.80}\\
\hline
Ours (vanilla) &No&point&25.18 &137.62 &0.37 &4.34\\
\rowcolor{Gray}
Ours &No&point&21.93 &136.80 &0.28 &3.98\\

\bottomrule
\end{tabular}}
\caption{\textbf{Effect of our approaches with point and box prompt on FSC-147.} \textbf{Bold} indicates the best counting results of training-free methods, and \underline{underline} indicates the best counting results of learning-based methods. \MM{missing arrow in MAE} 
}
\label{tab:box-prompt}
\end{table}


Even when using point prompts, our method still achieves remarkable results, significantly surpassing the two training-free baseline methods. We did not compare them to learning-based methods as they are unable to accommodate point prompts. Additionally, we observed that the results obtained by our method through point prompts are slightly inferior to those obtained through box prompts. This is because the mask of reference objects obtained using box prompts is more accurate, thereby improving the quality of the similarity map.

%
\begin{table}[!t]
\centering
\resizebox{0.99\columnwidth}{!}{
\begin{tabular}{@{}lccccccccccccc@{}}
\toprule
&\multirow{2}{*}{\textbf{Training}} & \multirow{2}{*}{\textbf{Prompt}} & \multicolumn{4}{c}{\textbf{CARPK}}\\
\cmidrule(lr){4-7}
& & & \textbf{MAE} $\downarrow$  &
\textbf{RMSE} $\downarrow$ & \textbf{NAE} $\downarrow$ &
\textbf{SRE} $\downarrow$ &  \\
\hline
GMN \cite{lu2019class} &Yes&box&7.48 &9.90 &- &-\\
FamNet+ \cite{ranjan2021learning} &Yes&box&18.19 &33.66 &- &-\\
BMNet+ \cite{shi2022represent} &Yes&box&\underline{5.76} &\underline{7.83} &- &-\\
SAM &No&N.A.&16.97 &20.57 &0.70 &5.30\\
Ours (vanilla) &No&box&15.47 &19.48 &0.69 &5.14\\
\rowcolor{Gray}
Ours &No&box&\textbf{10.97}&\textbf{14.24} &\textbf{0.48} &\textbf{3.70}\\
\hline
Ours (vanilla) &No&point&15.67 &19.44 &0.67 &5.06\\
\rowcolor{Gray}
Ours &No&point&11.01 &14.34 &0.51 &3.89\\

\bottomrule
\end{tabular}}
\caption{\textbf{Effect of our approaches with point and box prompt on CARPK.} Our methods are able to perform as well as the best learning-based method.
}
\label{tab:carpk}
\end{table}
